Curve-Induced Dynamical Systems on Riemannian Manifolds and Lie Groups

Deploying robots in household environments requires safe, adaptable, and interpretable behaviors that respect the geometric structure of tasks. Often represented on Lie groups and Riemannian manifolds, this includes poses on SE(3) or symmetric positive definite matrices encoding stiffness or damping. In this context, dynamical system-based approaches offer a natural framework for generating such behavior, providing stability and convergence while remaining responsive to changes in the environment. We introduce Curve-induced Dynamical systems on Smooth Manifolds (CDSM), a real-time framework for constructing and coupling motion profiles directly on Riemannian manifolds and Lie groups. The proposed approach constructs a nominal curve on the manifold, and generates a dynamical system which combines a tangential component that drives motion along the curve and a normal component that attracts the state toward the curve. We provide a stability analysis of the resulting dynamical system and validate the method quantitatively. We leverage the phase, indicating the progression along the curve, firstly, to define a phase modulation layer, that can modulate the timing while keeping a fixed spatial profile, and secondly, to couple dynamical systems and curves on different manifolds. We showcase the coupling's applicability in robot-assisted shoulder rehabilitation, and a real-world dressing task on both a robotic manipulator, where poses on SE(3) and damping matrices on SPD(n) are adapted online, and on a mobile manipulator. In quantitative evaluations on S2 and in robot-assistive tasks, CDSM demonstrates its effectiveness while achieving real-time curve-generation and fast query times.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();
push @sub_doc_options, '-pdf';

push @file_not_found, '^No file\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if ( $root_filename ne $_[0] ) {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;

        my $return = system "latexmk",
            @sub_doc_options,
            "-aux-directory=$sub_doc_output",
            "-output-directory=$sub_doc_output",
            $base_name;

        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
            rdb_add_generated( "$sub_doc_output/$base_name.aux" );
            copy "$sub_doc_output/$base_name.aux", ".";
        }

        popd;
        return $return;
    }
}
